Self-Calibrating Gaussian Splatting for Large Field of View Reconstruction

In this paper, we present a self-calibrating framework that jointly optimizes camera parameters, lens distortion and 3D Gaussian representations, enabling accurate and efficient scene reconstruction. In particular, our technique enables high-quality scene reconstruction from Large field-of-view (FOV) imagery taken with wide-angle lenses, allowing the scene to be modeled from a smaller number of images. Our approach introduces a novel method for modeling complex lens distortions using a hybrid network that combines invertible residual networks with explicit grids. This design effectively regularizes the optimization process, achieving greater accuracy than conventional camera models. Additionally, we propose a cubemap-based resampling strategy to support large FOV images without sacrificing resolution or introducing distortion artifacts. Our method is compatible with the fast rasterization of Gaussian Splatting, adaptable to a wide variety of camera lens distortion, and demonstrates state-of-the-art performance on both synthetic and real-world datasets.

==> images/supp_crop_fov220.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt} % Adjust space between columns if needed
    \begin{tabular}{cc} % 5 columns
        \includegraphics[height=0.2\textwidth]{images/fov220/4J9C8785_crop.jpg} &
         \includegraphics[height=0.2\textwidth]{images/fov220/4J9C8785_mask_crop.jpg} \\

        \multicolumn{1}{c}{(a) Original} & \multicolumn{1}{c}{(b) Cropped}
    \end{tabular}

    \caption{\textbf{Preprocessing of Ultra Wide Angle}. Meike camera we used has a FOV of 220\si{\degree}, which means it project scenes on the back of images plane. In this case, our first step of estimating extrinsic will fail in COLMAP~\cite{schoenberger2016sfm}}

    \label{fig:fov220}

\end{figure}
}

==> images/teaser.tex <==
\twocolumn[
\begin{figure*}[h]
    \centering
    % set the space between columns
    \setlength{\tabcolsep}{0.1em} 
    \renewcommand{\arraystretch}{0.75}
    \begin{tabular}{ccccc}
        \includegraphics[height=0.195\textwidth]{images/teaser/gt.jpg} &  
        \includegraphics[height=0.195\textwidth]{images/teaser/vanilla.jpg} &  
        \includegraphics[height=0.195\textwidth]{images/teaser/fisheye-gs.jpg} &  
        \includegraphics[height=0.195\textwidth]{images/teaser/ours.jpg} &  
        \includegraphics[height=0.195\textwidth]{images/teaser/gt_.jpg} \\
        (a) Ground truth full-image. & 
        (b) Vanilla GS &
        (c) ADOP &
        (d) Ours &
        (e) Ground truth.
    \end{tabular}
    \vspace{-1em}
    \caption{
    We introduce Bundle-Adjusting Gaussian Splatting, a differentiable rasterization pipeline that can produce high-quality view-synthesis results from imperfect camera parameters. 
    (b) Vanilla Gaussian Splatting~\cite{kerbl20233d} struggles with lens distortion because of the pinhole camera assumption. 
    (c) Existing self-calibration methods like ADOP~\cite{ruckert2022adop} fails to accurately represent complex distortions of lenses, leading to blurry rendering. 
    (d) Our model produces high-fidelity novel-view synthesis results by jointly modeling 3D scene representations, camera parameters, and lens distortion.
    }
    \label{fig:teaser}
\end{figure*}
]


==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\guandao}[1]{\textbf{\color{cyan}[guandao: #1]}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}
\usepackage{xcolor}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{float}
\usepackage{multicol}
\usepackage{tikz}
\usepackage{comment}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage[nopar]{lipsum}
\usepackage{stfloats}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{amsfonts}
\usepackage{siunitx}
\usepackage{stfloats}
\usepackage{etoolbox}
\usepackage{tocloft}
\usepackage{setspace}

\usepackage{color}
\usepackage{subcaption}
\usepackage[misc]{ifsym}

\usepackage{array}     % For tabular formatting and \arraystretch
\usepackage{caption}   % For handling captions
\usepackage{tabularx}  % Optional, for advanced table control

% \usepackage{orcidlink}
\usepackage{xcolor}
\usepackage{paralist}
% \usepackage{xltxtra}
\usepackage[capitalize]{cleveref}
% Support for easy cross-referencing
\usepackage{afterpage}

\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

\newcommand{\proj}[1]{\operatorname{proj}(#1)}
\newcommand{\homo}[1]{\operatorname{homo}(#1)}
\newcommand{\interp}[1]{\operatorname{interp}(#1)}
\newcommand{\fpp}[2]{\frac{\partial #1}{\partial #2}}

==> sec/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


==> tables/ablation_cubemap_vs_single_planar.tex <==
{
\begin{table}[t]

  \centering
  \scalebox{1}{
    \begin{tabular}{cccc}
    \toprule
    % \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} & \multicolumn{3}{c}{Image Metric}\\
    Method
    % \multicolumn{1}{c}{} 

    & PSNR  & SSIM  & LPIPS\\
    \midrule
    Small FOV Perspective     &19.08&0.654&0.332\\
    Ours (Single Planar)    &24.10&0.676&0.312\\
    Ours (Cubemap) &\textbf{29.01}&\textbf{0.792}&\textbf{0.253}\\
    \bottomrule
    \end{tabular}
  }
  \caption{\textbf{Ablation}}.
  \label{tab:ablation_cubemap_single}
\end{table}
}

==> tables/quantitative_mitsuba.tex <==
{\begin{table}[t]
  
  \centering
    \scalebox{1}{
    \begin{tabular}{cccc}
    \toprule
    % \multicolumn{1}{c}{\multirow{2}[2]{*}{Method}} & \multicolumn{3}{c}{Image Metric}\\
    Method
    % \multicolumn{1}{c}{} 
    & PSNR  & SSIM  & LPIPS\\
    \midrule
    Vanilla-GS~\cite{kerbl20233d}     &25.37&0.923&0.121\\
    % Fisheye-GS~\cite{liao2024fisheye}    &25.65&0.886&0.096\\
    % \midrule
    Ours &\textbf{28.00}&\textbf{0.932}&\textbf{0.093}\\
    \bottomrule
    \end{tabular}
    }
  \caption{\textbf{Quantitative Evaluations on Our Synthetic Dataset}}.
\label{tab:quantitative_mitsuba}
\end{table}}
